Studying the role of named entities for content preservation in text style transfer

Text style transfer techniques are gaining popularity in Natural Language Processing, finding various applications such as text detoxification, sentiment, or formality transfer. However, the majority of the existing approaches were tested on such domains as online communications on public platforms, music, or entertainment yet none of them were applied to the domains which are typical for task-oriented production systems, such as personal plans arrangements (e.g. booking of flights or reserving a table in a restaurant). We fill this gap by studying formality transfer in this domain. We noted that the texts in this domain are full of named entities, which are very important for keeping the original sense of the text. Indeed, if for example, someone communicates the destination city of a flight it must not be altered. Thus, we concentrate on the role of named entities in content preservation for formality text style transfer. We collect a new dataset for the evaluation of content similarity measures in text style transfer. It is taken from a corpus of task-oriented dialogues and contains many important entities related to realistic requests that make this dataset particularly useful for testing style transfer models before using them in production. Besides, we perform an error analysis of a pre-trained formality transfer model and introduce a simple technique to use information about named entities to enhance the performance of baseline content similarity measures used in text style transfer.

==> drafts.tex <==
% \begin{table}[t!]
% \small
% \centering
% \begin{tabular}{p{0.4\linewidth}p{0.2\linewidth}p{0.2\linewidth}}
% \toprule
% Metric & w/o NER & w NER \\ 
% \midrule
% MIS & \textbf{0.70} & 0.68 \\ 
% cross-stsb-large & \textbf{0.66} & 0.65 \\ 
% cross-stsb-base & 0.61 & \textbf{0.63} \\ 
% NUBIA & 0.60 & \textbf{0.61} \\ 
% \bottomrule
% \end{tabular}
% \caption{Spearman correlation of automatic content preservation metrics with human content preservation scores with and without using auxiliary NER-based metric on DSTC dataset}
% \label{tab:ner_experiments}
% \end{table}

% https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9628032
% https://arxiv.org/pdf/2109.13141v1.pdf

% Second, we try to enhance the cross-encoder architecture with NER-specific information. We use additional NER-specific embedding layer (each token was granted with either entity specific NER index or with zero index if it is not related to any entity). The similar idea is used in Med-BERT~\citet{liu2021med}. We also try to apply two forward passes of cross encoder: one with all tokens and another with all but Named entities tokens masked (similarly to~\citet{roy2021knowledge}) and then concatenate last hidden states of CLS tokens for predictions. 
% We use various combination of the aforementioned tools for creating the NER-oriented metric architecture. We train and test the model on isolated splits of our dataset. Even though this setting looked promising, none of the NER-information enriched architecture demonstrates significant improvement in comparison with the standard cross-encoder architecture. %The stratification of the phrases was performed according to the author of the initial phrase (system or client)




% Thus we make a conclusion that even though named entities are important for content preservation tracking, this can be handled reasonably by automatic metrics. 

% First, we took 313 pairs which have similarity score less or equal to 0.67 and check how often are entities really lost or corrupted if the pair of sentences is marked as non similar. It turns out that in 35\% of cases new sentence had one or more entity lost, in 27\% an entity is somehow corrupted (i.e. incorrectly paraphrased) and in 38\% no entities are affected, even though the sentence pair was ranked as non-similar. 




% We use domain-specific spans from the original SGD for training a NER tagger which is then used for extracting entities. These entities are processed with lemmatization, normalization (e.g. adjust `p.m.' and `pm' to the common form), entity linking, and then used to calculate the Jaccard index~\cite{jaccard_index} over the intersection between entities from an original and generated sentence. As shown on Tab.~\ref{tab:amr_mis_results}, this metric, if it is used separately, poorly correlates with human scores, but we observe that the more entities are in the pair, the higher this correlation can be (e.g. up to 0.6 on a subset of the SGD-based dataset with four or more entities per phrase), so we try to use it as an auxiliary signal for `strong' metrics (with the highest correlation).

% We apply some pre-processing to the tagged tokens: lemmatization, normalization of some regular entities (e.g. adjust 'p.m.' and 'pm' to the common form) and entity linking where applicable (e.g. the trained GYAFC-based style transfer model tends to paraphrase some entity names into more informal way, like 'New York' to 'NY'). We then measure the Jaccard index over raw or pre-processed tokens and over the collected entity ids and use it as metric for content preservation. It turns out that this metric has pretty low Spearman correlation with human scores - 0.16, but we observe that the more entities are in the original phrase the higher this correlation can be (up to 0.6), so we try to use it as an auxiliary signal for metrics with highest correlation with human scores. 

% According to the collected insights, we decide to stop experiments in this direction and make the conclusion that the top-performing metrics can naturally handle NER-specific information. We add the NER-based metric to our final report in \cref{fig:correlations_para,fig:correlations_tst} for consistency.
%and there is no need to explicitly embed it into architecture of a model. 
